On the Uniqueness of Solution for the Bellman Equation of LTL Objectives

Surrogate rewards for linear temporal logic (LTL) objectives are commonly utilized in planning problems for LTL objectives. In a widely-adopted surrogate reward approach, two discount factors are used to ensure that the expected return approximates the satisfaction probability of the LTL objective. The expected return then can be estimated by methods using the Bellman updates such as reinforcement learning. However, the uniqueness of the solution to the Bellman equation with two discount factors has not been explicitly discussed. We demonstrate with an example that when one of the discount factors is set to one, as allowed in many previous works, the Bellman equation may have multiple solutions, leading to inaccurate evaluation of the expected return. We then propose a condition for the Bellman equation to have the expected return as the unique solution, requiring the solutions for states inside a rejecting bottom strongly connected component (BSCC) to be 0. We prove this condition is sufficient by showing that the solutions for the states with discounting can be separated from those for the states without discounting under this condition

==> backup.tex <==
@article{oura_learning-based_2022,
	title = {Learning-Based Bounded Synthesis for Semi-{MDPs} With {LTL} Specifications},
	volume = {6},
	issn = {2475-1456},
	url = {https://ieeexplore.ieee.org/document/9762370},
	doi = {10.1109/LCSYS.2022.3169982},
	pages = {2557--2562},
	journaltitle = {{IEEE} Control Systems Letters},
	author = {Oura, Ryohei and Ushio, Toshimitsu},
	urldate = {2023-10-25},
	date = {2022},
	note = {Conference Name: {IEEE} Control Systems Letters},
}
@inproceedings{bozkurt_model-free_2021,
	title = {Model-Free Learning of Safe yet Effective Controllers},
	url = {https://ieeexplore.ieee.org/document/9683634},
	doi = {10.1109/CDC45484.2021.9683634},
	eventtitle = {2021 60th {IEEE} Conference on Decision and Control ({CDC})},
	pages = {6560--6565},
	booktitle = {2021 60th {IEEE} Conference on Decision and Control ({CDC})},
	author = {Bozkurt, Alper Kamil and Wang, Yu and Pajic, Miroslav},
	urldate = {2023-10-25},
	date = {2021-12},
	note = {{ISSN}: 2576-2370},
}

A button strongly connected component (BSCC) of an MC is a strongly connected component without outgoing transitions. 

Let $R: S\to\mathbb{R}$ be a reward function and  
let $\Gamma: S\to (0,1]$ be a state-dependent discount factor function of MDP $\mathcal{M}$. 
The $K$-step return ($K\in \mathbb{N}$ or $K=\infty$) of a path from time $t\in \mathbb{N}$ is
\begin{align}
G_{t:K}(\sigma) = \sum_{i=0}^{K} R(\sigma[t+i])\cdot \prod_{j=0}^{i-1} \Gamma(\sigma[t+j]), 
G_{t}(\sigma) = \lim_{K\to\infty}G_{t:K}(\sigma).
\end{align}

The value function $V_\pi(s)$ is the expected return conditional on the path start at $s$ and act w.r.t. policy $\pi$, 
\begin{align}
V_\pi(s) = \mathbb{E}_{\sigma\sim\pi}[G_t(\sigma)\,|\,\sigma[t] =s].
\end{align}
The Bellman equation (BE) is a recursion for expected returns
\begin{align}
    V_\pi(s) = R(s) + \Gamma(s) \sum_{s'\in S}P_\pi(s,s') V_\pi (s'). 
\end{align}

\zt{is this paragraph necessary?}
The computation of the value function is essential in various planning algorithms as it serves as a valuable metric to improve the policy. This computation can be achieved through Monte Carlo simulations, but solving the BE is more cost-effective. It is worth mentioning that the BE may become ill-posed with multiple solutions due to a sate-dependent discount factor, causing the overall planning algorithm to collapse.

% The action-value function, $Q^\pi(s,a)$,  is the expected return if the path start at $s$, $\sigma[0]=s$, and takes action $a$, and act w.r.t. policy $\pi$ afterwo\akb{a}rds. 
% \begin{align}
% Q^\pi(s,a) = \mathbb{E}_{\sigma \sim \pi}[G_t (\sigma)\,|\,s_0=s,a_0=a]
% \end{align}

% \section{Staisifcation Probability Recovery}


% we divide the expected return of a random path $\sigma$ from a state $s^\times$ by whether it visits the states $B$ infinitely often:

% \begin{align}
%     V (s) &= \mathbb{E}_\pi[G_t(\sigma,0)|\sigma[t]=s, \sigma \models \square \lozenge B] \mathbb{P}(s\models \square \lozenge B) \nonumber\\
%     &+ \mathbb{E}_\pi[G_t(\sigma,0)|\sigma[t]=s, \sigma \nvDash \square \lozenge B] \mathbb{P}(s\nvDash \square \lozenge B)
% \end{align}

% same as the proof to Lemma1, we have 
% $$
% \mathbb{E}_\pi[G_t(\sigma,0)|\sigma[t]=s, \sigma \models \square \lozenge B] = 1
% $$
% Then we have 
% $$V (s)\ge \mathbb{P}(s\models \square \lozenge B)$$

% Let $m$ denoting the number of state $s\in B$ visite before reaching a rejecting BSCC. 
% $$\mathbb{E}_\pi[G_t(\sigma,0)|\sigma[t]=s, \sigma \nvDash \square \lozenge B]
% \\
% = \mathbb{E}_\pi[1-\gamma^m|\sigma[t]=s, \sigma \nvDash \square \lozenge B]
% $$
% we have 
% \begin{align}
%     V(s) = \mathbb{P}(s\models \square \lozenge B) + (1-\gamma^{m'}) \mathbb{P}(s\nvDash \square \lozenge B)
% \end{align}


% From the above equality, since our method measures the exact probability upper bound, unlike csrl. 
% If we use two different discount factors to do the value function estimation in parallel, we can recover the true probability. 
% Given two different discount factor $\gamma_1$, $\gamma_2$
% \begin{align}\label{eqn:trueP}
%     V^{\gamma_1}(s) 
%     &= \mathbb{P}(s\models \square \lozenge B) + (1-{\gamma_1}^{m'}) \mathbb{P}(s\nvDash \square \lozenge B)  \nonumber\\
%     &=1-{\gamma_1}^{m'} \mathbb{P}(s\nvDash \square \lozenge B)  \nonumber\\
%     V^{\gamma_2}(s)&=1-{\gamma_2}^{m'} \mathbb{P}(s\nvDash \square \lozenge B)  \nonumber \\
%     {m'} &=\log_{(\frac{\gamma_1}{\gamma_2})} \frac{1-V_\pi^{\gamma_1}(s)}{1-V_\pi^{\gamma_2}(s)} \nonumber\\
%     \mathbb{P}(s\vDash \square \lozenge B) &= 1- \frac{1-V_\pi^{\gamma_1}(s)}{\gamma_1^{m'}}
% \end{align}
% In this way, the true satisfaction probability will be recovered and we can do a Q-learning based on the true probability. 
% \begin{theorem}
%     Given product MDP, reword with counter, and two discount factors $\gamma_1$,$\gamma_2$, the true satisfaction probability can be recovered by comparing the two parallel value functions $V_\pi^{\gamma_1}(s)$, $V_\pi^{\gamma_2}(s)$. 
% \end{theorem}

% A product MDP with reward and cost is defined as
% $ M^{\times} = ( S^{\times} , {\mathcal{LA}}^{\times} , P^{\times},s_0^{\times}) $.
% It's the product of the original $\mathcal{M} = ( S, {\mathcal{LA}}, P, s_0,AP, L)$, and an LDBA ${\mathcal{LA}}= (\mathcal{Q},\Sigma,\delta,q_0,B)$. 
% % augmented with additional LTL induced cost function $(C,\Gamma)$. 
% $S^\times = S \times \mathcal{Q}$ is the set of states, 
% ${ {A}}^\times = { {A}} \cup { {A}}^\epsilon, { {A}}^\epsilon:=\{\epsilon_q|q\in \mathcal{Q}\}$ is the set of actions, 
% $P^\times : S^\times \times  {A}^\times  \times S^\times \to [0,1]$ is the transition probability function,  
% \begin{align}
% &P^\times(\langle s,q\rangle,a,\langle s',q'\rangle) \notag
% \\&= \left \{
% \begin{array}{rcl}
% P(s,a,s')  &  &q'=\delta(q,L(s)) \,{\rm and}\, a\notin { {A}}^\epsilon \\
% 1             &  &a=\epsilon_{q'}\, {\rm and} \, q'\in \delta(q,\epsilon) \, {\rm and} \, s=s'\\
% 0             &  &{\rm otherwise}.
% \end{array}\right.
% \end{align}

% Reward and discount, 

% \begin{equation}
% R_{B}:=\begin{Bmatrix}
% 1-\gamma_{B} & s\in B \\ 
% 0 & s\notin B \\ 
% \end{Bmatrix},  \Gamma_{B}(s):=\begin{Bmatrix}
% \gamma_{B} & s\in B \\ 
% 1 & s\notin B \\ 
% \end{Bmatrix}
% \end{equation}
% Once a memoryless policy $\pi:s^\times\to A^\times$ is fixed, then we get an induced Markov Chain with an induced transition probability function. 
% \begin{align}
% P(\langle s,q\rangle, \langle s',q'\rangle) = P^\times(\langle s,q\rangle,\pi(\langle s,q\rangle),\langle s',q'\rangle)
% \end{align}
% For the induced transition probability $P:S^\times \times S^\times \to [0,1]$, we have the Bellman equation as, 

% \begin{equation}{\label{eqn:bellman}}
% \begin{Bmatrix}
% V(i) = 1-\gamma_{B}+\gamma_{B}\sum_{j\in S^\times}{P(i,j)V(j)}  & i\in B \\ 
% V(i) = \sum_{j\in S^\times}{P(i,j)V(j)}                         & i\notin B \\ 
% \end{Bmatrix}
% \end{equation}
% First, we define the set $S_B$ containing all $B$ states in the induced MC. The set $S_{\neg B}$ contains all $\neg B$ states in the induced MC. 
% Where $\vert S_B\vert =m$,$\vert S_{\neg B}\vert =n$. 
% $V_{B}\in\mathbb{R}^{m}$ is the vector listing the value function for all $s\in S_{B}$. 
% $V_{\neg  B}\in\mathbb{R}^n$ is the vector listing the value function for all $s\in S_{\neg B}$. 
% Given $\mathbb{I}$ as a column vector with all $1$ elements. Given $\mathbb{O}$ as a column vector with all $ 0$ elements. 
% We rewrite the above Bellman equation into vector form by partitioning the transition matrix $P^B_{ij}:=P^B(i,j)$ into four sub-matrices. 
% \zt{explain more for the notation}
% \begin{equation} \label{eqn:bellman vector}
% \begin{bmatrix}
% V_{B} \\ 
% V_{\neg B} \\ 
% \end{bmatrix} =(1-\gamma_{B})
% \begin{bmatrix}
% \mathbb{I}_{m} \\ 
% \mathbb{O}_{n} \\ 
% \end{bmatrix}
% +\begin{bmatrix}
% \gamma_{B}I_{m\times m} &   \\ 
%   & I_{n\times n} \\ 
% \end{bmatrix}
% \begin{bmatrix}
% P_{B\rightarrow B} & P_{B\rightarrow \neg B} \\ 
% P_{\neg B\rightarrow B} & P_{\neg B\rightarrow \neg B} \\ 
% \end{bmatrix}
% \begin{bmatrix}
% V_{B} \\ 
% V_{\neg B}
% \end{bmatrix}
% \end{equation}


\begin{example}
Consider a (product) MDP with two states $S = \{s_B, s_{\neg B}\}$ where $s_B$ is the initial state and the only accepting state, i.e., $B = \{s_B\}$.
Suppose under certain policy $\pi$, the transition probability is $1$ from $s_B$ to $s_{\neg B}$ and  $s_{\neg B}$ to itself, and $0$ otherwise, as shown in Figure \ref{fig:Ex1}. Then, the Bellman equation when setting $\gamma = 1$ is given below
% \zt{Suppose we have a MC induced from a product MDP by a policy}, it has one accepting state $s_B$ and one non-accepting state $s_{\neg B}$ as shown in Figure~\ref{fig:Ex1}, we can see the non-accepting state has a self-loop without any discounting. \yw{This is a MC not a LMDP}. The BE is written as, \zt{dicount = 1}
\zt{array to bmatrix}
\begin{align}
\begin{bmatrix}
V(s_B) \\ 
V(s_{\neg B}) \\ 
\end{bmatrix} = 
\begin{bmatrix}
1-\gamma_B \\ 
0\\ 
\end{bmatrix}+
\begin{bmatrix}
\gamma_{B}  &   \\ 
  & 1 \\ 
\end{bmatrix}
\begin{bmatrix}
0 & 1 \\ 
0 & 1 \\ 
\end{bmatrix}
\begin{bmatrix}
V(s_B) \\ 
V({s_{\neg B}}) \\ 
\end{bmatrix}. \label{eqn:Ex1}
\end{align}
The Bellman equation \eqref{eqn:Ex1} has multiple solutions because a value function of the form 
$$\begin{bmatrix}
V(s_B) & V({s_{\neg B}}) 
\end{bmatrix} = \begin{bmatrix}
1-\gamma_B +\gamma_B c & c 
\end{bmatrix}$$
with any $c \in \mathbb{R}$ is a solution.
% thus, any arbitrary constant can serve as the solution for $V(s_{\neg B})$. Correspondingly, $V(s_B)=1-\gamma_B +\gamma_B V(s_{\neg B})$. 
% \zt{When we set $\gamma_B=0.9$, then $V(s_{B})=c$, $V(s_{\neg B})=0.9c + 0.1$ serve as solution} 
\end{example}
% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \begin{tikzpicture}[>=stealth, node distance=2cm, on grid, auto]
% \node[initial,state, initial text={}] (A) {$s_B$};
% \node[state, right=of A] (B) {$s_{\neg B}$};

% \path[->]
% (A) edge[bend left] node {1} (B)
% (B) edge[loop right, min distance=10mm, in=30, out=60, looseness=8] node {1} (B);
% \end{tikzpicture}
% \caption{Example of a two-state Markov chain induced by a product MDP given some policy. The resulting Bellman equation \eqref{eqn:Ex1} has multiple solutions if we set $\gamma = 1$ in the surrogate reward \eqref{eqn:surrogate}.} \label{fig:Ex1}
% \end{wrapfigure}
% \zt{ask nathen for by and from} 

\subsubsection{Uniquness inside Accepting BSCCs}\label{sec:case1}
Inside a BSCC, every state is recurrent. For an accepting BSCC, at least one state in $B$ will be visited infinitely often. Any path inside the accepting BSCC will receive a total return as a geometric series $\sum_k^\infty{\gamma^k}=1$, which holds even if we discard all states in $\neg B$ and only look at the transition between states in $B$. Since on a non-accepting state $s\in{\neg B}$, no reward is collected, and no discount is applied to the future reward. The solution on $B$ seems independent of the solution on $\neg B$. 
\begin{proposition}\label{prop:1}
    For any accepting BSCC, the Bellman equation~\eqref{eqn:bellman vector} has a unique solution which is $\mathbb{I}$. 
\end{proposition}
Our approach to show this proposition relies on the transition between states in $B$ after we discard all states in $\neg B$. In the relation between states in $B$, $\gamma=1$ no longer appears and we can construct a new Bellman equation with the matrix $(I-\gamma_B P)$ invertible. 
However, the condition allows us to use only set $B$ to determine the solution of the Bellman equation~\eqref{eqn:bellman vector} does not come in for free. 
\begin{lemma}\label{lem:1}
    If the MC only has accepting BSCCs, then the Bellman equation~\eqref{eqn:bellman vector} has a unique solution $[V_B^T, V_{\neg B}^T]^T= \mathbb{I}$. 
\end{lemma}
An accepting BSCC is a closed, recurrent class inside an MC. And we can treat it as an independent MC without rejecting BSCCs. All the transition probabilities are still the same and the initial distribution does not matter since we are investing the value function for all states. 
Suppose Lemma~\ref{lem:1} holds, we can apply it to any accepting BSCC and show Proposition~\ref{prop:1} is true. 

We represent the transition between states inside $B$ by a new matrix $P_B$, where $P_B(i,j)$ stands for the probability of leaving the set $B$ at state $i$ and returning to the set $B$ at state $j$ without visiting any other state in $B$ between the leave and visit. 
\begin{align}\label{eqn:first return1}
P_B &:= P_{B\rightarrow B}+P_{B\rightarrow \neg B}\sum_{k=0}^\infty {P_{\neg B\rightarrow \neg B}^{k}}P_{\neg B\rightarrow B}. 
\end{align}
Inside this equation, we have the matrix power $P^k_{\neg B\to \neg B}$. Each element $(P^k_{\neg B\to \neg B})(i,j)$ represents the probability of a path leaving the state $i$ and visiting state $j$ after $k$ steps without travelling through any states in $B$. However, the absence of rejecting BSCCs ensures that any path will visit the a state in $B$ in finite times with probability $1$. Thus, we are sure $\forall i\in \neg B$, $\forall j \in \neg B$, $\sum_{k=0}^\infty(P^k_{\neg B\to \neg B})(i,j)=0$. This vanish of matrix power implies all eigenvalues of $P_{\neg B\to \neg B}$ are strictly within the unit disk which shows $(I - P_{\neg B\rightarrow \neg B})$ invertible. Thus we know the power series $\sum_{k=0}^\infty {P_{\neg B\rightarrow \neg B}^{k}}$ is bounded and~\eqref{eqn:first return1} can be rewritten as, 
\begin{align}\label{eqn:first return}
P_B =P_{B\rightarrow B}+P_{B\rightarrow \neg B} (I - P_{\neg B\rightarrow \neg B})^{-1}P_{\neg B\rightarrow B}.
\end{align}
$\forall i\in B$, $\forall j\in B$, $P_B(i,j)\ge 0$, the absence of rejecting BSCCs also ensures that $\forall i\in B$, $\sum_{j\in S} P_B(i,j)=1$. Thus, $P_B$ is a probability matrix that can be used to describe the behaviour of an MC with state space as $B$ only. 

\zt{this remark might be too important to be a remark, shall we call it a prop?}
\begin{remark}
Dropping all non-accepting states from the state space of induced MC $(S, P,s_0,\Lambda, L)$ allows us to build a new MC, which we call sub-MC $(B, P_B,\mu,\Lambda, L)$. 
The state space for the sub-MC is the set of accepting states $B$. The transition probability $P_B$ is the transition between all accepting states.
The initial distribution $\mu$ on the sub-MC is a distribution on $B$ and determined by $s_0$. 
\begin{align}
{\rm if}\,  s_0\in B,\quad   \lambda(s) =  
\begin{cases}
1 & s= s_0 \\ 
0 & s\ne s_0 
\end{cases},\quad
{\rm if}\,  s_0\notin B, \quad 
    \mu(s) = P_{init}(s_0,s)
\end{align}
where $P_{init} := (I-P_{\neg B\to \neg B})^{-1}P_{\neg B\to B}$ is a matrix representing the first visit to $B$ starting at $\neg B$. 
Since the absence of rejecting BSCC, we can construct a sub-MC, and every state will have a reward of $1-\gamma_B$ and a discount factor of $\gamma_B$. 
\end{remark}
\begin{lemma} 
    Suppose there is no rejecting BSCC, the Bellman equation~\eqref{eqn:bellman vector} is equivalent to the following form, 
\begin{align}\label{eqn:bellman case1}
\begin{bmatrix}
V_{B} \\ 
V_{\neg B} \\ 
\end{bmatrix} &=(1-\gamma_{B})
\begin{bmatrix}
\mathbb{I}_{m} \\ 
\mathbb{O}_{n} \\ 
\end{bmatrix} +\begin{bmatrix}
\gamma_{B}I_{m\times m} &   \\ 
  & I_{n\times n} \\ 
\end{bmatrix}\begin{bmatrix}
P_{B} &   \\ 
P_{\neg B\rightarrow B} & P_{\neg B\rightarrow \neg B} \\ 
\end{bmatrix}
\begin{bmatrix}
V_{B} \\ 
V_{\neg B} \\ 
\end{bmatrix}. 
\end{align}
\end{lemma}
\begin{proof}
We proof this lemman by showing showing the equivalence between $P_B V_B$ and $P_{B\to B}V_B + P_{B\to\neg B}V_{\neg B}$. 
From the Bellman equation~\eqref{eqn:bellman vector}, we have $V_{\neg B}=P_{\neg B\to B} V_B + P_{\neg B\to \neg B}V_{\neg B}$
\begin{align}
&P_{B\to B}V_B + P_{B\to\neg B}V_{\neg B}  \notag \\
&\overset{a}{=}(P_{B\to B}  + P_{B\to\neg B} P_{\neg B\to B}) V_B + P_{B\to\neg B} P_{\neg B\to \neg B}V_{\neg B}\notag\\
&\overset{b}{=}(P_{B\to B}  + P_{B\to\neg B} P_{\neg B\to B}  + P_{B\to\neg B}P_{\neg B\to \neg B} P_{\neg B\to B}) V_B + P_{B\to\neg B} P^2_{\neg B\to \neg B}V_{\neg B}\notag\\
&\vdots\notag\\
&\overset{c}{=}\lim_{K\to \infty}\big{(}(P_{B\to B}  + P_{B\to\neg B} \sum_{k=0}^K{P^k_{\neg B\to \neg B}} P_{\neg B\to B} )V_B + P_{B\to\neg B} P^{K+1}_{\neg B\to \neg B}V_{\neg B}\big{)} \notag \\
&\overset{d}{=}P_{B}V_B .
\end{align}
The equality $a$, $b$, $c$ hold as we keep expending $V_{\neg B}$. The equality $d$ holds by the definition of $P_B$.
\end{proof}
The equation~\eqref{eqn:bellman case1} claims that the solution $V_B$ is independent of the non-accepting states, providing a basis for showing its uniqueness. Subsequently, we leverage the dependence of $V_{\neg B}$ on $V_B$ to establish the uniqueness of the overall solution $V$.
\renewcommand{\proofname}{Proof for Lemma~\ref{lem:1}}
\begin{proof}
From equation~\eqref{eqn:bellman case1}, we obtain the expression for the sub-MC with only accepting states, 
\begin{equation}\label{eqn:sub-MC}
V_{B} =(1-\gamma_{B})\mathbb{I} +\gamma_{B}P_{B}V_{B}.
\end{equation}
Given that all eigenvalues of $P_B$ are within the unit disk and $\gamma_B<1$, the matrix $(I-\gamma_B P_B)$ is invertible. $V_B$ is uniquely determined by
\begin{align}\label{eqn:VB}
    V_B = (1-\gamma_{B})(I-\gamma_B P_B)^{-1} \mathbb{I}.
\end{align}
Moving to the set of non-accepting states $V_{\neg B}$, 
from equation~\eqref{eqn:bellman case1} we have, 
\begin{align}\label{eqn:neg B}
V_{\neg B} &= P_{\neg B\rightarrow B}V_{B}+P_{\neg B\rightarrow \neg B}V_{\neg B} \notag \\
&=(I-P_{\neg B\rightarrow \neg B})^{-1}P_{\neg B\rightarrow B}V_{B}.
\end{align}
Given the uniqueness of  $V_B$, and the invertibility of $(I-P_{\neg B\rightarrow \neg B})$, we conclude that $V_{\neg B}$ is also unique. 

Let $V_B=\mathbb{I}_m$ and $V_{\neg B}=\mathbb{I}_n$, the Bellman equation~\eqref{eqn:bellman vector} holds as the summation of each row of a probability matrix is always one, 
\begin{align} 
\begin{bmatrix}
\mathbb{I}_m \\ 
\mathbb{I}_n \\ 
\end{bmatrix} &=(1-\gamma_{B})
\begin{bmatrix}
\mathbb{I}_{m} \\ 
\mathbb{O}_{n} \\ 
\end{bmatrix} +\begin{bmatrix}
\gamma_{B}I_{m\times m} &   \\ 
  & I_{n\times n} \\ 
\end{bmatrix}\begin{bmatrix}
P_{B\rightarrow B} & P_{B\rightarrow \neg B} \\ 
P_{\neg B\rightarrow B} & P_{\neg B\rightarrow \neg B} \\ 
\end{bmatrix}
\begin{bmatrix}
\mathbb{I}_m \\ 
\mathbb{I}_n \\ 
\end{bmatrix}. 
\end{align}
Therefore, in the absence of rejecting BSCCs, the unique solution to the Bellman equation~\eqref{eqn:bellman vector} is $\mathbb{I}$.
\end{proof}

==> intro-old.tex <==
\section{Introduction}
\zt{outline

Why use LTL for RL?

    RL with LTL objective is an automatic way to design a reward function for an agent to learn.
    
    1. manually designing the reward function can be difficult, without performance guarantees. 
    
    2. using LTL to auto-design reward functions using less human labor, with a performance guarantee. 

What's the challenge if we use LTL objective for RL?

    1. Estimation Error embedded in discount factor. 
        the result is an upper bound for the satisfaction probability, there is always an error. 
        
    2. Slow convergence due to discount factor. 
        RL convergence reply on the discount factor $\gamma$ it's polynomial to the reciprocal of $1-\gamma$, taking the limit of $\gamma\to 1$ makes the convergence slow. 
        
    3. Sample complexity due to transition probability. (PAC-learnable) 

How does this work address the estimation error issue? 

    inspired by stochastic shortest-path problems and reachability problems. 
    
How does this work address the slow convergence due to the discount factor? 

How does this work explain the PAC-learnable? 

    whereas \cite{yang_tractability_2022} uses a specially crafted counter-example. Our work shows the general connection between convergence rate and transition probability.
}

Reinforcement Learning (RL) has shown its ability to let an agent learn complex tasks. 
However, if we want to specify a complex task to an agent, designing a proper reward function is often hard and tedious. To address this issue, a way to translate the desired behavior automatically into a reward function has been used. That is we encode the desired tasks into a Linear Temporal Logic (LTL) formula and then use some way to translate the LTL formula into a reward function. 

Several parallel works in 2020 serve as the foundation for many existing works \cite{oura_learning-based_2022,bozkurt_model-free_2021,cai_modular_2021,bozkurt_secure_2021,hasanbeig_certified_2023}  using LTL to generate reward functions for RL. Among these, the {CSRL} is the most popular one. However, {CSRL} suffers from the slow convergence rate and the estimation error on satisfaction probability inherently embedded in its discount factors. There has been a discussion on whether we should use a fully expressable LTL formula to assign tasks in RL.

In this work, we want to address these two problems by directly confronting the compromise people used to make to discount factors. We are not going to take the limit of a discount factor to one, that's the reason for slow convergence. And we are going to directly treat the other discount factor as one, that's the reason causing the estimation error. 

Taking the discount factor as one would cause problems like lacking a convergence guarantee and even resulting in multiple fixed points for the Bellman equation. And that's the reason why {CSRL} and {MC} didn't remove the discount factors even though it would remove the estimation error. 

On the other track, there is a doubt of whether an LTL formula is PAC learnable. In the \cite{yang_tractability_2022}, a specially crafted counter-example is proposed to show the sample complexity for an LTL RL algorithm depending on a choke point in the Markov Chian. In this work, we will provide a convergence rate analysis rely on the transition matrix and it will work for the general Markov Chain. This would give us a better understanding of what we like about environment, and applying LTL objective can be PAC learnable. 









% More recently, people have begun to use the learning approach to incorporate formal objectives in planning\cite{hahnOmegaRegularObjectivesModelFree2019}.
% Building a product MDP is a common approach. It \akb{what does "it" refer to?} requires \akb{to} transform a formal logic into an automaton, combine the automaton with the MDP to construct a product MDP. This is an approach \akb{that} has been used for decades, but recently people are incorporating more powerful \akb{"powerful" might be confusing here as LDBAs' expressive power is the same as NBAs.} automantion \akb{automata?} such as Limit-Deterministic B\"uchi Automata \akb{we can cite the papers describing how to construct an LDBA} \cite{bozkurt2020controlb,bozkurt2021modelfreee,bozkurt2021modelfreed}. New \akb{maybe just "LDBAs"} automata allows us to \akb{allow for the use of} use the fully expression of a LTL formular \akb{a bit confusing} to serve as the objective for the planning in MDP. 

\subsection{CSRL like result} 
Here we show how previous works evaluate the policy. 
Given a product MDP with accepting $B$ states, given a memoryless policy $\pi$, evaluate the satisfaction probability $P (\sigma | \sigma[0]=s, \sigma \models \square \lozenge B)$ which is the probability of all paths run on the induced MC, start at state $s$ and satisfy $\sigma \models \square \lozenge B$. 

Multiple approaches to solving the above problem formulation rely on building a reward $R_B(s)$ and discount $\Gamma(s)$ structure and thus making the corresponding Bellman equation's solution close to the satisfaction probability. 

\zt{I can have two versions here, one using BSCC and one avoid using BSCC}

The intuition behind this reward structure is straightforward. Along a path, a constant reward will be collected only on the accepting state. Suppose the discount factor $\gamma=1$, infinitely often visiting the accepting states will result in a summation of a geometric series equal to one. The satisfaction probability on whether a path will infinitely often visit the accepting states will be equal to how likely such a geometric series summation will be constructed along a path. 


But in the general scenario, the BE solution $V  (s)$ under this reward structure will not be the exact satisfaction probability $P(s\models \square \lozenge B)$. 
\begin{align}
    V  (s) &= \mathbb{E} [G_t(\sigma)|\sigma[t]=s, \sigma \models \square \lozenge B] P(s\models \square \lozenge B) \nonumber\\
    &+ \mathbb{E} [G_t(\sigma)|\sigma[t]=s, \sigma \nvDash \square \lozenge B] P(s\nvDash \square \lozenge B)
\end{align}

For a path $\sigma$ satisfies $\square \lozenge B$, having discount factor $\gamma<1$ will result in additional discounting that makes the return $G_{t}(\sigma)$ less than the summation of a geometric series. That is $\mathbb{E} [G_t(\sigma)|\sigma[t]=s, \sigma \models \square \lozenge B]<1$. 
For a path $\sigma$ that visits accepting states finitely often but not zero times, having $\gamma_B<1$ and the return $G_{t}(\sigma)$ will be positive instead of zero. That is $\mathbb{E} [G_t(\sigma)|\sigma[t]=s, \sigma \nvDash \square \lozenge B]>0$.

Several approaches have been introduced to mitigate the error brought by discount factors. 

\zt{$\gamma_B(\gamma)$ needs def} 
\begin{theorem}
For a given product MDP with $B\subseteq S$, with the surrogate reward structure~\eqref{eqn:surrogate}, the value function $V $ for policy $\pi$ satisfies 
\begin{align}
    \lim_{\gamma\to 1^-} V ^\gamma(s)=P(s\models \square \lozenge B)
\end{align}
for all state $s\in S$. If  $\gamma_B(\gamma)$ in~\eqref{eqn:surrogate} is a function of $\gamma$ satisfies
\begin{align}
    \lim_{\gamma\to 1^-} \frac{1-\gamma}{1-\gamma_B(\gamma)}=0
\end{align}
\end{theorem}

The main theorem used in [][][] trying to make the BE solution close to the satisfaction probability, however, the prerequisite on the discount factors is strict. Taking the discount factor's limitation up to $1^-$ will result in slow convergence in the computation. As in dynamic programming, the contraction is guaranteed by discount factor $<1$, and in RL, the convergence rate is upper bounded by a polynomial of the reciprocal of $1-\gamma$ [][][]. 

Recently there have also been other approaches trying to directly take $\gamma = 1$ [][]. It seems the error brought by  $\mathbb{E} [G_t(\sigma)|\sigma[t]=s, \sigma \models \square \lozenge B]<1$ can be canceled, however, we can see this approach will introduce new problems. 

The most straightforward shortcoming comes as the convergence guarantee breaks. The convergence guarantee for the Q-learning used in [][] needs a discount factor always $<1$. We know there are convergence guarantee for cases [] when discount factor can be one, but they need additional treatment. \zt{how should I support this claim, write down a stochastic approximation for RL convergence seems too cumbersome here}


\yw{Good example. Need to articulate. And go after the Bellman Equation}
Another issue along with the convergence is that the BE may have multiple solutions. 
Here is a trivial example, 
\zt{try to move BE (14) and this counterexample before problem formulation}
